WarpNet: Weakly Supervised Matching for Single-view Reconstruction

We present an approach to matching images of objects in fine-grained datasets without using part annotations, with an application to the challenging problem of weakly supervised single-view reconstruction. This is in contrast to prior works that require part annotations, since matching objects across class and pose variations is challenging with appearance features alone. We overcome this challenge through a novel deep learning architecture, WarpNet, that aligns an object in one image with a different object in another. We exploit the structure of the fine-grained dataset to create artificial data for training this network in an unsupervised-discriminative learning approach. The output of the network acts as a spatial prior that allows generalization at test time to match real images across variations in appearance, viewpoint and articulation. On the CUB-200-2011 dataset of bird categories, we improve the AP over an appearance-only network by 13.6%. We further demonstrate that our WarpNet matches, together with the structure of fine-grained datasets, allow single-view reconstructions with quality comparable to using annotated point correspondences.

==> Source/derivetps.tex <==
\section{Computing TPS Coefficients}
\label{sec:TPS}
Given a regular grid points $\{\bm{x}_i\}$ and deformed grid points $\{\bm{x}'_i\}$,  $i = 1, \dots, K^2$, the TPS transformation from the regular grid coordinate frame to the deformed grid coordinate frame for the $x$-coordinates is given by
\begin{align}
  T_{\theta_x}(\bm{x}) &= \sum_{j = 0}^3 a^x_j\phi_j(\bm{x}) +
  \sum_{i=1}^{K^2}w^x_i U(||\bm{x}, \bm{x}_i||),   \label{eq:1} \\
\text{s.t.}\quad& \sum_{i=1}^{K^2}w^x_i = 0,\quad  \sum_{j=1}^2\sum_{i=1}^{K^2}w^x_ix_j = 0,\nonumber
\end{align}
where $\phi_0 = 1$,  $\phi_j(\bm{x}_i) = x_j$, $U(r) = r^2\log r^2$. A similar transformation may be expressed for the $y$-coordinate, denoted $T_{\theta_y}(\bm{x})$, with coefficients $\bm{w}^y$ and $\bm{a}^y$. The final transformation is $T_\theta(\bm{x}) = [T_{\theta_x}(\bm{x}), T_{\theta_y}(\bm{x})]$. With the interpolation conditions $T_\theta(\bm{x}_i) = \bm{x}'_i$, we can write the TPS coefficients $\theta =
\begin{pmatrix}
  \bm{w}^x & \bm{w}^y\\
  \bm{a}^x & \bm{a}^y
\end{pmatrix}$ as the solution to a system of linear equations:
\begin{equation}
\label{eq:linsys}
L \theta = \begin{pmatrix}
  \bm{x}' \\ 0
  \end{pmatrix},
\end{equation}
where
$ L = \begin{pmatrix} K & P \\ P^T & 0 \end{pmatrix}$, $K_{ij} = U(||\bm{x}_i - \bm{x}_j||)$ and row $i$ of $P$ is $(1, x_i, y_i)$. As discussed in \cite{bookstein}, $L$ is non-singular, invertible and only needs to be computed once, since the regular grid $\bm{x}$ is fixed for our application. Thus, computing the TPS coefficients from a deformed grid is a linear operation $\theta = L^{-1}\bm{x}'_i$ with weights, $L^{-1}$, computed once in the beginning of the training. 


